Tables Decoded: DELTA for Structure, TARQA for Understanding

Table understanding is a core task in document intelligence, encompassing two key subtasks: table reconstruction and table visual question answering (TabVQA). While recent approaches predominantly rely on vision- language models (VLMs) operating on table images, we propose a more scalable and effective alternative based on structured textual representations. These representations are easier to process, align more naturally with LLMs, and eliminate the need for language-specific visual encoders, making them particularly suitable for multilingual documents. We present DELTA, which separates physical structure recognition, logical structure recognition, and OCR to extract both layout and content accurately. DELTA outputs tables in Optimised Table Structure Language (OTSL), a compact and unified format that encodes cell arrangements and textual content. On table structure recognition (TSR), DELTA achieves TEDS- Structure scores comparable with state-of-the-art methods across FinTabNet, PubTabNet, and PubTables-1M. We further establish its robustness on non-English tables through our curated Hindi benchmark, TORQUE. Building on this, we introduce TARQA, an LLM fine-tuned on OTSL sequences. Our approach yields gains of 9.3 p.p. on WTQ (TabQA) and 9.2 p.p. on FinTabNetQA (TabVQA), respectively. On TORQUE, our method ranks second among all VLMs and DELTA + LLM variants. We release our code, models, and benchmark at: https://github.com/Tihiitborg/Tables-Decoded

==> R1_Archive/sec/0_abstract.tex <==
\begin{abstract}
% Table understanding is a key task in document intelligence, with table reconstruction and table question answering being two of its most important associated tasks. While some recent models use table images as input to vision language models (VLMs), we argue that converting tables into structured text sequences is a more effective and scalable alternative. Textual representations are easier to process, align well with the capabilities of existing LLMs, and avoid the need for language-specific visual encoders, making them especially suitable for multilingual documents. We propose \textit{\name}, a structured table reconstructor that uses the minimized Optimized Table Structure Language (OTSL) as a unified representation for both structure and content. OTSL encodes logical relationships such as cell arrangements, row and column spans, and hierarchy in a compact sequence format that preserves both structural and semantic information. Our reconstruction pipeline converts input table images into HTML, and then lossless OTSL conversion is performed on it, achieving high alignment with ground truth as measured by TEDS scores on benchmarks including FinTabNet, PubTabNet, and PubTables-1M. Additionally, when OTSL-formatted tables generated by \textit{\name{}} are used as input prompts for LLMs, we observe significant improvements in table-based question-answering tasks. We release the code and models to promote reproducibility and facilitate further research in multilingual and structure-aware table understanding.

Table understanding is a core task in document intelligence, encompassing two key subtasks: table reconstruction and table visual question answering (TabVQA). While recent approaches predominantly rely on vision-language models (VLMs) operating on table images, we propose a more scalable and effective alternative based on structured textual representations. These representations are easier to process, align more naturally with large language models (LLMs), and eliminate the need for language-specific visual encoders, making them particularly suitable for multilingual documents. We present \name, a decoupled table reconstruction framework that separates structure recognition from OCR to extract both layout and content accurately. \name{} outputs tables in Optimized Table Structure Language (OTSL), a compact and unified format that encodes cell arrangements and textual content. \name{} achieves high-fidelity table-to-text conversion, outperforming prior methods on structure metrics with superior TEDS-Structure scores across FinTabNet, PubTabNet, and PubTables-1M. On FinTabNet, it surpasses the best VLM baseline by an absolute 0.4\% in overall TEDS score. Built on \name, we introduce \tabqa{} (Table structure-Aware Representation for Question Answering), an LLM fine-tuned on OTSL-formatted tables for accurate and structure-aware TabVQA. \tabqa{} outperforms HTML-based models by 14.2\%, and improves answer accuracy on WTQ by 6.8\% and on FinTabNetQA by 9.2\%. We release our code and models to advance research in multilingual, structure-aware table understanding.

\end{abstract}


==> R1_Archive/sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Tables are a key format for conveying structured information across domains like science, finance, and administration. Their visual structure encodes relational data, making table understanding essential for recovering layout and content. This is crucial for downstream tasks such as retrieval, parsing, summarization, and TabVQA. However, real-world table documents pose significant challenges. They exhibit diverse layouts ranging from simple grids to deeply nested hierarchies, with variations in formatting, font, language, and visual cues. Merged cells, multi-row or multi-column spans, empty placeholders, and handwritten or low-quality scans introduce additional complexity. Broadly, as seen in Figure \eqref{fig:teaser}, existing approaches to table understanding follow one of the two distinct paradigms. The first relies on VLMs, which directly consume table images and jointly model visual and textual features using transformer-based architectures pretrained on large-scale multimodal datasets. These models are typically fine-tuned end-to-end for tasks such as table detection, reconstruction, or TabVQA. 

\begin{figure*}
    \centering
    \fbox{\includegraphics[width=\linewidth]{sec/figures/teaser.pdf}}
    \caption{Two paradigms for TabVQA: the end-to-end paradigm uses a VLM to directly process the table image and question, while the decoupled paradigm extracts structure and content via TSR and OCR, converts it into a textual format (e.g., HTML, OTSL), and then uses an LLM for answering. Our approach follows the decoupled paradigm for better control and multilingual support.}
    \label{fig:teaser}
\end{figure*}

The second paradigm leverages LLMs, which operate entirely in the language space. In this setting, tables are first serialized into textual formats such as HTML, Markdown, LaTeX, or plain-text formats before being provided as input prompts to LLMs (Figure \eqref{fig:teaser}). The models then reason over these serialized tables to answer questions or perform related tasks. While VLMs benefit from strong visual grounding, they are often monolithic and inflexible, tightly coupling layout reasoning, content extraction, and question answering into a single opaque pipeline. This end-to-end dependency makes them difficult to debug or adapt. Moreover, they require extensive pretraining with image-text pairs. VLMs also show a performance gap, especially for non-Latin scripts or low-resource languages. Crucially, the internal representations they learn are often not interpretable or easily transferable to new tasks. In contrast, LLM-based approaches offer a modular, language-agnostic alternative by separating the concerns of table recognition and reasoning. Once tables are converted into structured textual formats, general-purpose LLMs can perform downstream tasks like TabVQA with minimal fine-tuning. However, the challenge lies in the table serialization process itself. An important factor that significantly impacts table understanding performance, especially when leveraging LLMs, is the choice of table representation. Simple plain-text formats fail to preserve structural information such as rows, columns, and cells, making it difficult for models to infer relationships between table elements. While formats like LaTeX and HTML can accurately capture table structures, they are often verbose and lead to long token sequences, which strain the input limitations of most LLMs and reduce overall efficiency. Markdown, though more compact, cannot faithfully represent complex structures involving merged cells, making it unsuitable for documents with complex tables. These limitations highlight the need for a compact format, one that preserves both structure and content while remaining well-suited for LLM-based processing. To address this, we advocate the use of the recently proposed OTSL sequences \cite{otsl}. OTSL provides a minimal yet expressive linear representation of tables, encoding hierarchical layouts, cell spanning, and cell-level textual content in a format that is significantly shorter than HTML while maintaining structural integrity. We propose a modular pipeline that uses Table Structure Recognition (TSR) and Optical Character Recognition (OCR) to extract table structure and content, which are serialized into the OTSL format. This decoupled approach offers interpretability and robustness across diverse document styles and languages. It outperforms recent VLM-based end-to-end methods on standard benchmarks and provides a scalable foundation for TabVQA. By shifting reasoning to text-based LLMs over OTSL, our method naturally extends to multilingual TabVQA, including low-resource scripts. Our main contributions can be summarized as follows:

\begin{itemize}
    \item Firstly, we present \name{}, a decoupled table reconstruction framework that performs TSR followed by OCR, producing a compact OTSL representation that achieves high structural fidelity on popular benchmarks, outperforming recent VLMs.
    
    \item Second, to support downstream tasks, we introduce an algorithm to convert widely used HTML formats into OTSL, effectively capturing both structure and content. 
    
    \item Finally, we propose \tabqa{}, an LLM fine-tuned on OTSL-formatted tables for TabVQA, showing strong performance over models fine-tuned on HTML and other baselines on WTQ and FinTabNetQA datasets.
\end{itemize}


Section \eqref{sec:Related work} reviews related work on VLMs and decoupled TSR + OCR-based approaches. In Section \eqref{sec: Table Reconstruction}, we describe the methodology behind \name{} and \tabqa{} in detail. The experimental setup is presented in Section \eqref{sec:experiments}, and the results are discussed in Section \eqref{sec:Results}. Finally, we conclude and outline future directions in Sections \eqref{sec:conclusion} and \eqref{sec:future}, respectively.

==> R1_Archive/sec/2_related_work.tex <==
\section{Related Literature}
\label{sec:Related work}

\textbf{End-to-End Table Reconstruction} leverages VLMs for holistic table understanding, aiming to directly generate structured representations such as HTML or JSON from table images. These models utilize pre-trained vision-language encoders to jointly process visual and textual cues, enabling end-to-end prediction of table structures, including cell relationships and content. Approaches like MTLTabNet \cite{mtl-tab-net}, SmolDocLing \cite{nassar2025smoldocling}, SmolVLM \cite{smolvlm}, and Granite-Vision \cite{granitevision} fall into this category. The key advantage of this paradigm is its ability to unify structure and content prediction without relying on intermediate OCR outputs or handcrafted rules. However, these models often struggle with multilingual scripts, complex layouts, and noisy scanned documents, particularly when such variations are underrepresented in training data.

\textbf{Decoupled Table Reconstruction} involves two key steps: TSR and OCR. TSR models are responsible for identifying cell boundaries, spanning relationships, and table skeletons. Object detection-based TSR methods focus on reconstructing the physical layout of tables by localizing cells using models like Faster R-CNN \cite{faster-rcnn}, Mask R-CNN \cite{mask-rcnn}, YOLO \cite{yolo}, etc. Transformer-based variants such as DETR \cite{detr, tatr-pub-1m}, TableFormer \cite{tableformer}, and TSRFormer \cite{tsrformer3} have also been equipped for this task. However, such object detection-based TSR often depend on post-processing for mapping cells to row and column numbers, making them sensitive to detection errors. Later, Im2Seq-based TSR methods dominated the field of TSR, where they directly predict the logical structures (cell mapping) from images using encoder-decoder architectures, outputting formats like HTML or LATEX. Recent approaches adopt compact representations like OTSL \cite{otsl, kudale2025sprint} to improve inference efficiency and structural consistency. Hybrid TSR methods, including graph-based models like GTE \cite{gte} and TGRNet \cite{tgrnet}, treat table reconstruction as a graph problem, mapping cell relations as edges. Others combine visual detection with token-level generation, such as multi-decoder attention models \cite{tsr-local-attention}, or use visual and positional cues to refine predictions \cite{lgpma, tabstruct, vast}. The emergence of Im2Seq models has often offered better end-to-end consistency by synchronizing physical and logical structure predictions in a unified pipeline. Table reconstruction datasets such as PubTabNet \cite{edd}, FinTabNet \cite{fintabnet}, PubTables \cite{tatr-pub-1m}, SynthTabNet \cite{synthtabnet}, and TabRecSet \cite{tabrecset} provide diverse annotations, with evaluation metrics like TEDS \cite{edd} and GriTS \cite{grits} assessing both spatial and structural accuracy. Once the structure is extracted, OCR engines are used to recognize the textual content within each cell.  Popular OCR engines suitable for this task include Tesseract \cite{tesseract}, DocTR \cite{doctr}, and several others \cite{surya, easyocr, paddleocr}. 

\textbf{Table-based Question Answering} (TabQA) focuses on reasoning over structured table data, typically provided in CSV or HTML format, to answer natural language questions. Recently, LLMs \cite{grattafiori2024llama, jiang2024mixtral, qwen} have been fine-tuned or prompted for direct reasoning over tabular inputs, exhibiting strong zero-shot and few-shot capabilities. However, their performance heavily depends on the quality and format of both the table and the prompt. Thus, the choice of representation used to encode tabular data becomes a critical design decision in decoupled TableVQA pipelines. TableVQA, in contrast, integrates visual understanding with question answering, operating directly on document images that contain tables. As discussed earlier, there are two main approaches to TableVQA \cite{kim2024tablevqa_bench}: (i) VLM-based models \cite{hu2024mplug_docowl, llava, blip2, qwen, cogagent, wang2023cogvlm} that jointly encode visual and textual information to generate answers, and (ii) decoupled pipelines that first extract table structure and content via TSR + OCR, then apply LLMs for textual question answering. We build upon this paradigm, where \name{} handles the decoupled table reconstruction, followed by \tabqa{} for question answering. Both components of our approach are detailed in the upcoming  Section \eqref{sec: Table Reconstruction}.

==> R1_Archive/sec/3_tab_rec.tex <==
\section{Our Methodology}
\label{sec: Table Reconstruction}
To enable structured understanding and question answering over tables, our methodology is divided into two main components: \name{}, which generates an OTSL sequence from input table images, and \tabqa{}, a TabVQA model fine-tuned on OTSL sequences. Figure \eqref{fig:tarka-pipeline} presents an overview of our proposed pipeline. The right half of the figure provides a brief illustration of our \name{} methodology: given a table image, we perform TSR followed by OCR to extract the table content. The widely used HTML representation is then transformed into an OTSL sequence in a lossless manner using our presented Algorithm \ref{algo_html_to_otsl}. The figure further demonstrates the use case of \tabqa{}, where the OTSL sequence generated by \name{} is used as input for inference. Overall, our methodology for \name{} consists of the following key steps, which we elaborate on in the subsequent subsections:

% \begin{figure*}
%     \centering
%     \begin{subfigure}[t]{\textwidth}
%         \centering
%         % trim={<left> <bottom> <right> <top>}
%         \fbox{\includegraphics[width=0.96\linewidth]{sec/figures/startle1.pdf}}
%         \caption{The pipeline begins by converting a table image into an HTML sequence using \name. This HTML representation is then losslessly transformed into a structured OTSL (Optical Table Structure Language) sequence, preserving both the semantic and spatial layout of the table. The OTSL format enables accurate table reconstruction and serves as a reliable input for downstream tasks such as table-based question answering.}
%         \label{fig:method1}
%     \end{subfigure}%
%     \vfill
%     \vspace{0.5cm}
%     \begin{subfigure}[t]{\textwidth}
%         \centering
%         % trim={<left> <bottom> <right> <top>}
%         \fbox{\includegraphics[width=0.96\linewidth]{sec/figures/qa.pdf}}
%         \caption{Given an input table image, our approach first converts it into a structured OTSL  sequence using \name. This OTSL representation captures the table’s semantic and structural layout in a text-based format. The resulting OTSL sequence is then passed to \tabqa{}, alongside the user query. \tabqa{} performs reasoning over the structured representation to accurately generate the answer corresponding to the query.}
%         \label{fig:method2}
%     \end{subfigure}
%     \caption{Overview of our proposed method. (a) the OTSL generation pipeline, and (b) the downstream table QA process.}
%     \label{fig:method_combined}
% \end{figure*}

\begin{figure*}[]
    \centering
    \fbox{\includegraphics[width=0.63\textwidth]{sec/figures/DELTA-TARK.pdf}}
    \caption{Overview of the \tabqa{} pipeline. Given a document image and a natural language query, the system first performs TSR, followed by OCR to extract table content. The resulting HTML is converted into a compact OTSL sequence. \tabqa, an LLM fine-tuned on OTSL, uses this structured input along with the query to generate accurate answers, enabling robust TabVQA.}
    \label{fig:tarka-pipeline}
\end{figure*}

\subsection{TSR for Cell Demarcation}
For TSR, we employ a combination of SPRINT \cite{kudale2025sprint} and TATR \cite{smock2023aligning}, which together provide a comprehensive understanding of table layouts. We chose SPRINT as it has shown fast, robust, and language-agnostic performance on logical TSR, making it ideal for capturing cell relationships across diverse scripts. TATR, also a recent state-of-the-art model, complements this by focusing on physical structure recognition, accurately identifying rows and columns to demarcate individual cells in the table image. The combined output is a structured HTML tag sequence that represents the table, including complex features such as cell merges, row spans, and column spans, with each \texttt{<td>} tag annotated with precise bounding box coordinates. The output of the TSR step with cells highlighted is seen in Figure \eqref{fig:tarka-pipeline}.

\subsection{OCR for Content Extraction}
The output of the TSR step, namely, the HTML tag sequence with bounding box annotations, is then used to perform OCR on each cell. We utilize Tesseract \cite{tesseract} for this task due to its broad support for multiple languages, modularity, and ease of integration. For each \texttt{<td>} tag, the corresponding bounding box is used to crop the cell region from the original table image, and Tesseract extracts the textual content from it. This text is then embedded back into the HTML string, enriching the structural representation with content-level information. Tesseract will enable seamless extension to multilingual tables.
The final HTML sequence, which preserves both the structure and the extracted content after the OCR step, is illustrated in Figure \eqref{fig:tarka-pipeline}. 


\subsection{HTML to OTSL conversion}
As highlighted in prior work \cite{otsl}, HTML representations are often large and noisy due to their verbose and repetitive tag structures, making them suboptimal for direct use with LLMs in TabQA tasks. To overcome these limitations, we convert the HTML output into an OTSL sequence, a compact, structured format that efficiently captures both the table’s layout and content. This conversion significantly reduces input length while preserving all necessary information, making it more suitable for LLM-based inference and leading to improved performance. We present Algorithm \eqref{algo_html_to_otsl}, which outlines the process of converting a content-rich HTML sequence into its corresponding OTSL representation in a lossless manner. Figure \eqref{tab_rep} provides an example of a complex table, showcasing the HTML generated by our TSR, followed by the OCR approach and the resulting OTSL sequence. This comparison demonstrates the compactness and structured clarity of OTSL, which enhances downstream task performance. We refer readers to the original OTSL specification \cite{otsl} for a detailed understanding of its syntax and token design.

 
\begin{algorithm}
\caption{Extract OTSL Matrix from HTML string}
\begin{algorithmic}[1]
\Require HTML string
\Ensure OTSL matrix string

\State Parse HTML, find \texttt{<table>}
\State Compute $R$ (rows) and $C$ (columns) using \texttt{rowspan}, \texttt{colspan}
\State Initialize $\text{otsl\_matrix}[R][C] \gets \texttt{"<ecel>"}$
\State Initialize $\text{cell\_map}[R][C] \gets 0$

\For{each row $i$}
    \State $col\_idx \gets 0$
    \For{each cell in row}
        \While{$\text{cell\_map}[i][col\_idx] = 1$} \State $col\_idx \gets col\_idx + 1$ \EndWhile
        \State Extract $rowspan$, $colspan$, text
        \State Assign \texttt{"<fcel>"} if text exists, else \texttt{"<ecel>"}
        \State Fill merged cells: \texttt{"<lcel>"} (left), \texttt{"<ucel>"} (up), \texttt{"<xcel>"} (cross)
        \State Update $\text{cell\_map}$, move to next column
    \EndFor
\EndFor

\State Convert $\text{otsl\_matrix}$ to string with \texttt{"<nl>"} separators
\State \Return OTSL matrix 

\end{algorithmic}
\label{algo_html_to_otsl}
\end{algorithm}


% In this section, we first introduce the syntax of the OTSL language, followed by a detailed description of the \name{} architecture. We then present the lossless conversion algorithm that translates HTML into OTSL sequences.



% \subsection{Significance of OTSL}

% The OTSL (Optimised Table Structure Language) is a linearized representation designed to encode table structures in a compact and model-friendly format. Each token in OTSL corresponds to a specific type of table cell or structural marker. The following tokens define the core syntax of OTSL:
% \begin{enumerate}
% \vspace{-3pt}
%     \item \texttt{<ecel>}: Represents an empty cell, indicating that the cell contains no textual content.
% \item \texttt{<fcel>}: Denotes a filled cell with textual content.
% \item \texttt{<lcel>}: Indicates a left-referenced cell, typically used for cells that span multiple columns and reference the left neighbor.
% \item \texttt{<ucel>}: Indicates an up-referenced cell, used when a cell spans multiple rows and refers to the cell above.
% \item \texttt{<xcel>}: Represents a cross-referenced cell, which is part of both row and column spans and is linked to both the cell above and the one to the left.
% \item \texttt{<nl>}: A row separator token used to indicate the end of the current row and the start of a new one.
% \end{enumerate}




% \subsection{Model Architecture}

% The proposed model adopts an \textit{encoder-decoder} architecture tailored for visually grounded table understanding and question-answering. 

% Subsequently, the generated OTSL string is fed into a separate, decoupled decoder alongside the user query. This final stage is responsible for producing the answer corresponding to the query grounded in the table structure. An overview of the complete model architecture is illustrated in Figure \eqref{fig:method_combined}.


% \begin{table*}[htbp]
% \renewcommand{\arraystretch}{1.3}
% \centering
% \begin{tabular}{
%     p{2cm}  % Training Stage
%     p{2cm}  % Tasks
%     p{4.5cm}  % Prompt
%     p{3cm}  % Target Sequence
%     p{1.5 cm}  % Parsed Datasets
%     p{1cm}  % Dataset Images
% }
% \toprule
% \textbf{Training Stage} & \textbf{Tasks} & \textbf{Prompt} & \textbf{Target Sequence} & \textbf{Datasets} & \textbf{\# of Images} \\
% \midrule
% \textbf{Pre-training} & Table Reconstruction & 
% \texttt{<s><image>Image Embedding</image> <ocr> SEQUENCE </s>} & 
% OTSL Representation for Structure and Content & 
% PubTables,\linebreak FinTabNet,\linebreak PubTabNet & 
% 1.4 M \\
% \bottomrule
% \textbf{Fine-Tuning} & Table Question Answering & 
% \texttt{<s> Instruction \linebreak OTSL string \linebreak Question \linebreak Answer </s>} &
% % \#\#\# Instruction: 
% % Given the following table, answer the question in one word or a short phrase. Do not provide an explanation.\linebreak
% % \#\#\# Table: \linebreak
% % \{table\_text\} \linebreak
% % \#\#\# Question: \linebreak
% % \{question\} \linebreak
% % \#\#\# Answer:\linebreak \{answer\} </s>} & 
% Answer to the input question & 
% Wiki Table Questions (WTQ)& 
% 12 K \\
% \bottomrule
% \end{tabular}
% \caption{Tasks, prompts, and target sequence formats used at two stages of the model. Special tokens \texttt{<s>} and \texttt{</s>} denote sequence boundaries, while \texttt{<image>} and \texttt{</image>} indicate the start and end of image embeddings.}
% \label{prompt_tab}
% \end{table*}


% \subsubsection{Loss function}



\begin{figure}[h]
\centering

% ---- Left: Table Grid ----
\begin{minipage}[t]{0.3\textwidth}
\centering
\begin{tikzpicture}


% Draw grid with equal row heights
\draw (0,0) rectangle (3,2);
\draw (0,1) -- (3,1);  % horizontal line separating ABC from bottom rows
\draw (1,1) -- (1,0);  % vertical line
\draw (2,1) -- (2,0);  % vertical line
\draw (1,0.5) -- (3,0.5);  % horizontal line dividing bottom rows equally

% Text
\node at (1.5,1.5) {\textbf{ABC}};
\node at (0.5,0.75) {\textbf{D}};
\node at (1.5,0.75) {\textbf{E}};
\node at (2.5,0.75) {\textbf{F}};
\node at (2.5,0.25) {\textbf{H}};
\end{tikzpicture}
\end{minipage}
\hfill

% First downward arrow with label
% \vspace{2mm}
\begin{center}
$\downarrow$ \hspace{0.3cm} \small Using Table Reconstruction
\end{center}
% \vspace{2mm}


% ---- Right: HTML ----
\begin{minipage}[t]{0.33\textwidth}
\centering
\begin{tcolorbox}[colback=white, colframe=black, boxrule=0.2mm]
\centering
\textit{\textbf{\textcolor{red}{HTML}}}

\vspace{2mm}
\small
\begin{tt}
<html><table><tr>\\
<td colspan=3>\textcolor{blue}{ABC}</td> </tr><tr><td rowspan=2>\textcolor{blue}{D}</td><td>\textcolor{blue}{E}</td>
<td>\textcolor{blue}{F}</td></tr><tr><td>
</td><td>\textcolor{blue}{H}</td>
</tr></table></html>
\end{tt}
\end{tcolorbox}
\end{minipage}

% Second downward arrow with label
% \vspace{0.1cm}
\begin{center}
$\downarrow$ \hspace{0.3cm} \small Using Algorithm \eqref{algo_html_to_otsl}
\end{center}
% \vspace{0.1cm}

% ---- Middle: OTSL ----
\begin{minipage}[t]{0.33\textwidth}
\centering
\begin{tcolorbox}[colback=green!10!white, colframe=black, boxrule=0.2mm]
\centering
\textit{\textbf{\textcolor{green!50!black}{Our Minimized OTSL}}}

\vspace{2mm}
\small
\begin{tt}
<otsl>\\
<fcel>\textcolor{blue}{ABC}<lcel><lcel><nl>\\
<fcel>\textcolor{blue}{D}<fcel>\textcolor{blue}{E}<fcel>\textcolor{blue}{F}<nl>\\
<ucel><ecel><fcel>\textcolor{blue}{H}<nl>\\
</otsl>
\end{tt}
\end{tcolorbox}
\end{minipage}
\hfill


\caption{Illustration of converting HTML sequence into OTSL sequence using Algorithm \ref{algo_html_to_otsl}.}
\label{tab_rep}
\end{figure}




==> R1_Archive/sec/4_exp_results.tex <==
\section{Experiments}
\label{sec:experiments}
Now that we have described \name{} for producing OTSL sequences, we proceed to validate the effectiveness of OTSL as the most suitable representation for TabQA (and eventually TabVQA). To this end, we conduct a series of experiments comparing OTSL with other common table representations, including HTML, 
% Markdown, 
and plain text. Our experimentation is structured as follows: we first describe the datasets used for these experiments, followed by a detailed explanation of the experimental setup, where LLMs are fine-tuned on each representation format to assess their impact on downstream TabQA performance. Finally, after establishing that OTSL yields the best performance for TabQA, we justify the use of \name{} in the pipeline and explain how its ability to generate high-quality OTSL sequences makes it well-suited for integration with the \tabqa{} model, thereby enabling more accurate TabVQA.

\subsection{Datasets}
We use three widely adopted datasets, FinTabNet, PubTabNet, and PubTables, to evaluate the performance of the \name{} pipeline on the table reconstruction task. We report the results on the validation split for the PubTabNet dataset. For this, we report TEDS-S and TEDS scores (Refer Table \eqref{tab:metric_definitions}), which measure structural fidelity and combined structure-content preservation, respectively. For the TabQA component, we utilize the WikiTableQuestions (WTQ) dataset to fine-tune LLMs for the TabQA task. We finetune LLMs with various table representations, namely HTML, 
% Markdown, 
plain text, OTSL, and report the performance of each on the WTQ test set. Based on these ablations, we identify the best-performing LLM, referred to as \tabqa{}. To evaluate the end-to-end TabVQA pipeline from table image to getting an answer, we use the FinTabNetQA dataset, which consists of approximately 205 table images along with 250 associated questions. Further details on the number of samples used from each dataset in our experiments are provided in Table \eqref{data_tab}.

\begin{table}
\centering
\begin{tabular}{lccc}
\hline
\textbf{Dataset} & \textbf{Train} & \textbf{Val} & \textbf{Test} \\
\hline
FinTabNet   & -  & - & 10305 \\
PubTabNet   & - & 6942 & -        \\
PubTables   & - & -  & 92841 \\
WTQ & 11321 & - & 7175\\
FinTabNetQA & - & - & 250\\
\hline
\end{tabular}
\caption{Dataset statistics for table reconstruction and TabQA.}
\label{data_tab}
\end{table}


\begin{table*}[ht]
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lp{11cm}}
\toprule
\textbf{Metric} & \textbf{Definition} \\
\midrule
\textbf{Tree Edit Distance-based Similarity (TEDS)} & Measures the similarity between predicted and ground truth HTML table structures using tree edit distance. It evaluates both the structure and content of tables, which we use to evaluate \name{} pipeline. \\
\textbf{TEDS-Structure (TEDS-S)} & A TEDS variant that evaluates only the HTML tag sequence, ignoring content. We use it to assess \name{}'s table structure recognition. \\
\textbf{Average Normalized Levenshtein Similarity (ANLS)} & Measures textual similarity between predicted and ground truth answers using the normalized Levenshtein distance, providing partial credit for near matches. We use this metric to evaluate \tabqa{} on the WTQ dataset. \\
% \textbf{EM (Exact Match)} & A strict binary metric that returns 1 if the predicted answer matches the ground truth exactly, and 0 otherwise. \\
\textbf{Relieved-Accuracy} & This metric considers predictions correct if any normalized form matches the ground truth, ignoring units and formatting. It emphasizes semantic equivalence and is used to evaluate \name{} + \tabqa{} on the FinTabNetQA dataset for the TabVQA task. \\
\bottomrule
\end{tabular}
}
\caption{Overview of metrics used for evaluating \name{} and \tabqa.}
\label{tab:metric_definitions}
\end{table*}


% We assessed our model on three prominent table structure datasets: FinTabNet, PubTabNet, and PubTables-1M. Table \eqref{data_tab} summarizes the dataset statistics, detailing the number of training, validation, and test samples for both table reconstruction and table question answering tasks. FinTabNet and PubTables provide structured HTML annotations, which are readily convertible to OTSL, while PubTabNet is primarily utilized for validation. To evaluate table reconstruction quality, we employed the Tree Edit Distance-based Similarity Structure (TEDS-S) and Tree Edit Distance-based Similarity (TEDS) score, which captures only structural and both structural as well as content-level alignment with the ground truth, respectively. For the downstream task, we used the WikiTableQuestions dataset, a large-scale resource for question answering on semi-structured tables. Model performance was measured using exact match accuracy (EM) and Levenshtein similarity ($\geq 0.8$) to assess answer quality.

% \begin{table}
% \centering
% \begin{tabular}{lccc}
% \hline
% \textbf{Dataset} & \textbf{Train} & \textbf{Val} & \textbf{Test} \\
% \hline
% Fintabnet   & 88{,}441  & 10{,}505  & 10{,}397 \\
% Pubtabnet   & 388{,}002 & 6{,}942   & -        \\
% Pubtables   & 751{,}027 & 93{,}989  & 92{,}841 \\
% WTQ & 11321 & - & 7175\\
% % Synthtabnet & 121{,}458 & 51{,}313  & 40{,}703 \\
% \hline
% \end{tabular}
% \caption{Dataset statistics for table reconstruction and Table Question Answering}
% \label{data_tab}
% \end{table}

\begin{table}[h]
\centering
\begin{tabular}{|c|c|}
\hline
\multicolumn{2}{|c|}{
\begin{minipage}[t]{0.3\textwidth}
\centering
\begin{tikzpicture}
\vspace{2pt}
% Draw grid with equal row heights
\draw (0,0) rectangle (3,2);
\draw (0,1) -- (3,1);
\draw (1,1) -- (1,0);
\draw (2,1) -- (2,0);
\draw (1,0.5) -- (3,0.5);

% Text
\node at (1.5,1.5) {\textbf{ABC}};
\node at (0.5,0.75) {\textbf{D}};
\node at (1.5,0.75) {\textbf{E}};
\node at (2.5,0.75) {\textbf{F}};
\node at (2.5,0.25) {\textbf{H}};
\end{tikzpicture}
\end{minipage}
} \\
\hline
Plain Text & ABD D E F H  \\ \hline
% Markdown   & \begin{tabular}[c]{@{}c@{}}\texttt{||||| --- | --- | --- |}\\\texttt{| ABC |||| D | E | F ||| H |}\end{tabular}      \\ \hline
HTML       & \begin{tabular}[c]{@{}c@{}}\textless{}tr\textgreater{}\textless{}td colspan="3"\textgreater{}ABC\\ \textless{}/td\textgreater{}\textless{}/tr\textgreater{}\textless{}tr\textgreater{}\textless{}td rowspan="2"\textgreater\\ D\textless{}/td\textgreater{}\textless{}td\textgreater{}E\textless{}/td\textgreater{}\textless{}td\textgreater{}F\textless{}/td\textgreater{}\textless{}/tr\textgreater\\ \textless{}tr\textgreater{}\textless{}td\textgreater{}\textless{}/td\textgreater{}\textless{}td\textgreater{}H\textless{}/td\textgreater{}\textless{}/tr\textgreater{}\end{tabular} \\ \hline
OTSL       & \begin{tabular}[c]{@{}c@{}}\textless{}fcel\textgreater{}ABC\textless{}lcel\textgreater{}\textless{}lcel\textgreater{}\textless{}nl\textgreater\\ \textless{}fcel\textgreater{}D\textless{}fcel\textgreater{}E\textless{}fcel\textgreater{}F\textless{}nl\textgreater\\ \textless{}ucel\textgreater{}\textless{}ecel\textgreater{}\textless{}fcel\textgreater{}H\textless{}nl\textgreater{}\end{tabular}                \\ \hline                                                    
\end{tabular}
\caption{Different table representations generated from the sample table input image.}
\label{tab:rep_formats}
\end{table}


\subsection{Generating Table Representations}
The WTQ training set already contains HTML sequences (ground truth). To create inputs in other formats, we apply format-specific conversions: for OTSL, we use our proposed Algorithm \eqref{algo_html_to_otsl} to convert the HTML into a compact sequence; and for plain text, we parse the HTML content row-wise (left to right) and flatten it into a simple text string. An illustration of these different formats is shown in Table \eqref{tab:rep_formats}. Based on the chosen representation format, the corresponding LLM is fine-tuned for the TabQA task.

\subsection{LLM Fine-tuning and Ablations}

We fine-tuned the Meta-LLaMA-3-8B-Instruct \cite{llama3modelcard} for the question-answering task to generate concise, accurate natural language answers based on a table OTSL sequence and a question. The model was fine-tuned using a custom instruction-tuned setup, where each example followed a structured prompt template that included an instruction, a serialized table, a natural language question, and the ground truth answer. 

\begin{small}
\begin{ttfamily}
\noindent
\#\#\# Prompt Used for Finetunung: \\
Given the following table, answer the question in one word or a short phrase. Do not provide an explanation.\\[1ex]
\#\#\# Table: \{OSTL\_sequence\}\\[1ex]
\#\#\# Question: \{User query\}\\[1ex]
\#\#\# Answer: \{answer\} \\
\end{ttfamily}
\end{small}


The WTQ dataset, in JSON format, was preprocessed using the HuggingFace AutoTokenizer with padding to a maximum sequence length of 4096 tokens and truncation enabled. The fine-tuning was conducted on an NVIDIA H100 80GB GPU using PyTorch and HuggingFace frameworks, with the AdamW optimizer and a learning rate of $2e^ {-5}$. Inference was performed using greedy decoding with the model. The effectiveness of OTSL as a representation format for TabVQA is demonstrated through our ablation study in Table \eqref{tab:rep_formats_ablation}, which compares different input formats across both off-the-shelf and fine-tuned LLMs, highlighting that fine-tuning using OTSL (\tabqa) led to the best scores. 

\begin{table}[]
\centering
\begin{tabular}{llcc}
\hline
\textbf{Format} & \textbf{LLM Model \cite{llama3modelcard}} & \multicolumn{1}{c}{\textbf{ANLS}} & {\textbf{EM}}\\ \hline
\multirow{2}{*}{OTSL}       & Off the Shelf  & 25.4	&16.9    \\
                            & Finetuned on OTSL                   & \textbf{56.5}	& \textbf{54.0 }            \\ \hline
\multirow{2}{*}{HTML}       & Off the Shelf                       &                                   11.0	& 10.3        \\
                            & Finetuned on HTML                   &     42.3	& 39.9                                 \\ \hline
% \multirow{2}{*}{Markdown}   & Off the Shelf                       &                                    26.69	& 25.05       \\
%                             & Finetuned on Markdown               &     72.51	& 70.59                                  \\ \hline
\multirow{2}{*}{Plain Text} & Off the Shelf                       &                                  29.8	& 27.8         \\
                            & Finetuned on Plain Text             &     52.8	& 50.2  \\ \hline                               
\end{tabular}
\caption{Comparing the impact of fine-tuning on different table representations on TabQA performance. For each format, we report scores from both off-the-shelf LLMs and those fine-tuned on the respective representation, showing that fine-tuning on OTSL results in an improvement of 14.2\% over fine-tuning on HTML.}
\label{tab:rep_formats_ablation}
\end{table}

% \begin{small}
% \begin{center}
% \begin{minipage}{0.9\linewidth}
% \begin{ttfamily}
% \noindent
% \#\#\# Instruction: \\
% Given the following table, answer the question in one word or a short phrase. Do not provide an explanation.\\[1ex]
% \#\#\# Table:\\
% \{table\_text\}\\[1ex]
% \#\#\# Question:\\
% \{question\}\\[1ex]
% \#\#\# Answer: \{answer\}
% \end{ttfamily}
% \end{minipage}
% \end{center}
% \end{small}



% \textcolor{red}{needs to be change according to our hyperparameter}
% \begin{table}[htbp]
% \centering
% \begin{tabular}{lcc}
% \hline
% \textbf{Hyperparameter}     & \textbf{Pre-training} & \textbf{Fine-tuning} \\
% \hline
% Training steps              & 415                   & -- \\
% Number of epochs            & 5                     & -- \\
% \multicolumn{2}{l}{Batch size}               & 128 \\
% \multicolumn{2}{l}{Optimizer}                & AdamW \\
% \multicolumn{2}{l}{Learning rate}            & 2.00E-04 \\
% \multicolumn{2}{l}{Learning rate decay}      & Linear \\
% \multicolumn{2}{l}{Adam $\beta$}             & (0.9, 0.98) \\
% \multicolumn{2}{l}{Weight decay}             & 0.01 \\
% \multicolumn{2}{l}{Dropout}                  & 0.1 \\
% \hline
% \end{tabular}
% \caption{Hyperparameters used during pre-training and fine-tuning}
% \end{table}


==> R1_Archive/sec/5_conclusion.tex <==
\section{Results and Discussions}
\label{sec:Results}

We evaluate the effectiveness of our approach, \name{}, across multiple table reconstruction benchmarks. \name{} generates HTML tag sequence strings, encompassing structure and content. As shown in Table \eqref{tab:metric_definitions}, we report the TEDS and TEDS-S scores of \name. Table \eqref{ted_table} compares \name{} with state-of-the-art methods on the FinTabNet, PubTabNet, and PubTables datasets using TEDS-S metrics. Our model demonstrates competitive performance in structural alignment, as evidenced by TEDS-S scores across all three datasets. TEDS scores for models evaluated on the FinTabNet dataset are presented in Table \eqref{tab:vlm_comparison_teds}. While \name{} outperforms VLMs in combined structural and content alignment with the ground truth, it lags behind approaches like VAST \cite{vast} and TableFormer \cite{tableformer}. This is primarily because those methods leverage PDF parsing for content extraction, resulting in near-perfect content fidelity, whereas we rely on OCR, which introduces performance bottlenecks. However, \name{} is modular, and replacing the OCR module with a more accurate one can significantly boost TEDS scores. Overall, these results underscore \name{}’s strong structural understanding and offer a clear path forward for improving content alignment.

% \begin{table*}[t]
% \centering
% \label{tab:vlm_comparison}
% \begin{tabular}{llcccccc}
% \toprule
% \textbf{Type} & \textbf{Approach} & \multicolumn{2}{c}{\textbf{FinTabNet}} & \multicolumn{2}{c}{\textbf{PubTabNet}} & \multicolumn{2}{c}{\textbf{PubTables}} \\
% \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
%  &  & \textbf{TEDS-S} & \textbf{TEDS} & \textbf{TEDS-S} & \textbf{TEDS} & \textbf{TEDS-S} & \textbf{TEDS} \\
% \midrule
% \multirow{4}{*}{\textbf{End-to-end VLMs}} 
% & SmolVLM\cite{smolvlm} & - & 18.0 & - & - & - & 32.0 \\
% & Granite-Vision\cite{granitevision} & - & 54.0 & - & - & - & 70.0 \\
% & MTL-TabNet\cite{ly2023end} & \textbf{98.8} & - & \textbf{97.9} & 96.7 & 96.7 & 96.2 \\
% & SmolDocling\cite{nassar2025smoldocling} & 81.0 & 52.0 & - & - & 65.0 & 88.0 \\
% \midrule
% \textbf{Decoupled Structure \&} & & & & & & & \\ 
% \textbf{Content Extraction} & \textbf{\name{}} & \textbf{98.2 }& \textbf{54.4} & \textbf{97.6} & 41.45 & \textbf{97.7} & ?? \\
% \textbf{through OCR} & & & & & & & \\
% \midrule

% {\textbf{Decoupled Structure \&}} & EDD\cite{zhong2019image}  + PDF Parsing & 90.6 & - & 89.9 & 88.3 & - & - \\
% {\textbf{Content Extraction}}& TableFormer\cite{tableformer}  + PDF Parsing & 96.8 & 89.0 & 96.75 & 93.6 & - & 84.0 \\
% {\textbf{through PDF Parsing}}& VAST\cite{huang2023improving} + PDF Parsing & \textbf{98.6} & 98.2 & 97.2 & 96.0 & - & - \\
% \bottomrule
% \end{tabular}
% \caption{Comparison of TEDS-S and TEDS metrics scores for different table reconstruction methods across three popular benchmarks: FinTabNet, PubTabNet, and PubTables-1M. Our method (\name) is evaluated alongside existing baselines, including both visual and hybrid approaches. Higher TEDS-S and TEDS scores indicate better structural alignment with ground truth.}
% \label{ted_table}
% \end{table*}

In Table \eqref{qa_tab}, we evaluate the impact of our structured outputs on the downstream TabQA task. We compare the performance of \tabqa{} using OTSL sequences generated by \name{} against other approaches on the WTQ test set. The results show that OTSL-based inputs lead to significantly higher QA accuracy, surpassing the strongest baseline by 6.8\%. We evaluate the performance of our integrated pipeline, \name{} + \tabqa{}, on the FintabnetQA dataset \cite{kim2024tablevqa_bench}. We compare our model's performance against various baselines, including both open and closed source VLMs. As shown in Table \eqref{table:fintabnetqa_scores}, our approach achieves higher relieved accuracy than all other baselines, showing the effectiveness of our pipeline. Figure \eqref{fig:qual} shows the qualitative results of \name{} and \tabqa{} on the TabVQA task. This superior performance highlights the pipeline's ability to enhance LLMs' adaptability for comprehending complex tables.   

\begin{table*}[]
\centering
\begin{tabular}{llccc}
\toprule
\textbf{Type} & \textbf{Approach} &{\textbf{FinTabNet}} &{\textbf{PubTabNet}} &{\textbf{PubTables}} \\
\midrule
\multirow{2}{*}{\textbf{End-to-end VLMs}} 
% & SmolVLM\cite{smolvlm} & - & - \\
% & Granite-Vision\cite{granitevision} & - & - & - \\
& MTL-TabNet\cite{ly2023end} & \textbf{98.8} & \textbf{97.9} & 96.7\\
& SmolDocling\cite{nassar2025smoldocling} & 81.0 & - & 65.0 \\
\midrule 

& EDD\cite{zhong2019image}  & 90.6 & 89.9 & - \\
\textbf{Decoupled Structure \&}& TableFormer\cite{tableformer}  & 96.8 & 96.8 & - \\
\textbf{Content Extraction}& VAST\cite{huang2023improving} & \textbf{98.6} & 97.2 & -  \\
 & \textbf{\name{} (Ours)} & \textbf{98.2 }& \textbf{97.6} & \textbf{97.7} \\
\bottomrule
\end{tabular}
\caption{Comparison of TEDS-S scores across three popular benchmarks: FinTabNet, PubTabNet, and PubTables}
\label{ted_table}
\end{table*}

\begin{table}[]
\centering
\begin{tabular}{lccc}
\toprule
\textbf{Baseline} &{\textbf{TEDS}} \\
\midrule
\multirow{3}{*}{End-to-end  VLMs} &
SmolVLM\cite{smolvlm} & 18.0 \\
& Granite-Vision\cite{granitevision} &54.0 \\
% & MTL-TabNet\cite{ly2023end} & \textbf{98.8} & - & \textbf{97.9} & 96.7 & 96.7 & 96.2 \\
& SmolDocling\cite{nassar2025smoldocling} &  52.0  \\
\midrule
Decoupled  & \textbf{\name{}} &  \textbf{54.4} \\
% \midrule
Structure \& &
*TableFormer\cite{tableformer}  & 89.0 \\
Content Extraction & *VAST\cite{huang2023improving} &  98.2 \\
 

\bottomrule
\end{tabular}
\caption{Comparison of TEDS metrics scores for different table reconstruction methods across FinTabNet showcasing 0.4\% improvement of TEDS over VLM-based approaches. Approaches marked by * use PDF-parsing for content extraction.}
\label{tab:vlm_comparison_teds}
\end{table}

\begin{table}
\centering
\begin{tabular}{lcc
    }
\hline
\textbf{Baseline} &  \textbf{WTQ} \\

\hline
UDOP\cite{tang2022unifying}  & 47.2  \\
Pix2struct\cite{lee2022pix2struct} &  39.8\\
DocOwl\cite{hu2024mplug_docowl}  & 26.9 \\
Kosmos\cite{peng2023kosmos2}  & 32.4 \\
Donut\cite{kim2021ocrfree}& 18.8\\
\textbf{\tabqa{}} & \textbf{54.0}\\
\hline
\end{tabular}
\caption{Comparison of ANLS scores on the WTQ dataset, evaluating \tabqa{} against pre-reported scores from other methods.}
\label{qa_tab}
\end{table}

% \begin{table}[]
%     \begin{center}
%         \resizebox{0.6\linewidth}{!}{%
%             \begin{tabular}{lc} \toprule
%             \textbf{Model} & \textbf{FinTabNetQA} \\ \midrule
%             % GPT-4V~\cite{gpt4v} & 79.6 \\
%             % Gemini-ProV~\cite{gemini} & 60.8 \\
%             SPHINX-MoE-1k & 36.0 \\
%             SPHINX-v2-1k & 31.2 \\
%             QWEN-VL-Chat~\cite{qwen} & 29.6 \\
%             QWEN-VL~\cite{qwen} & 34.0 \\
%             SPHINX-MoE & 2.8 \\
%             SPHINX-v1-1k~\cite{lin2023sphinx} & 3.2 \\
%             mPLUG-Owl2~\cite{ye2023mplug} & 2.8 \\
%             LLaVA-1.5~\cite{liu2023llava-1.5} & 0.8 \\
%             CogVLM-1k~\cite{wang2023cogvlm} & 4.8 \\
%             SPHINX-v1~\cite{lin2023sphinx} & 1.2 \\
%             CogAgent-VQA~\cite{cogagent} & 22.8 \\
%             InstructBLIP~\cite{instructblip} & 0.4 \\
%             BLIP-2~\cite{blip2} & 0.4 \\
%             CogVLM~\cite{wang2023cogvlm} & 1.2 \\
%             CogAgent-VQA~\cite{cogagent} & 22.8 \\
%             % GPT-4V~\cite{gpt4v} $\rightarrow$ GPT-4~\cite{gpt4} & 95.2 \\
%             % Gemini-ProV~$\rightarrow$~Gemini-Pro~\cite{gemini} & 75.6 \\
%             % GPT-4~\cite{gpt4} & 98.8 \\
%             % Gemini-Pro~\cite{gemini} & 96.4 \\
%             % GPT-3.5 & 93.2 \\
%             % Vicuna-13B~\cite{vicuna2023} & 84.8 \\
%             % Vicuna-7B~\cite{vicuna2023} & 68.8 \\
%             \textbf{\name{} + \tabqa{}} & \textbf{45.2} \\
%             \bottomrule
%             \end{tabular}
%         }
%     \end{center}
%      \caption{Accuracy score on FinTabNetQA different models v/s \textbf{Ours}.}
%      \label{table:fintabnetqa_scores}
% \end{table}


\begin{table}[]
    \begin{center}
        \resizebox{0.9\linewidth}{!}{%
            \begin{tabular}{llc}
                \toprule
                \textbf{Type} & \textbf{Model} & \textbf{FinTabNetQA} \\ \midrule
                \multirow{12}{*}{Open-source} 

                & BLIP-2~\cite{blip2} & 0.4 \\
                & InstructBLIP~\cite{instructblip} & 0.4 \\
                & CogVLM-1k~\cite{wang2023cogvlm} & 4.8 \\
                & CogAgent-VQA~\cite{cogagent} & 22.8 \\
                & CogVLM~\cite{wang2023cogvlm} & 1.2 \\
                & mPLUG-Owl2~\cite{ye2023mplug} & 2.8 \\
                & SPHINX-v1~\cite{lin2023sphinx} & 1.2 \\
                & SPHINX-v1-1k~\cite{lin2023sphinx} & 3.2 \\
                 & LLaVA-1.5~\cite{liu2023llava-1.5} & 0.8 \\
                & QWEN-VL-Chat~\cite{qwen} & 29.6 \\
                & QWEN-VL~\cite{qwen} & 34.0 \\
                 \cmidrule(lr){1-3}
                \multirow{3}{*}{Closed-source} 
                 & SPHINX-MoE-1k\cite{kim2024tablevqa_bench} & 36.0 \\
                & SPHINX-v2-1k\cite{kim2024tablevqa_bench} & 31.2 \\
                & SPHINX-MoE\cite{kim2024tablevqa_bench} & 2.8 \\
                \cmidrule(lr){1-3}
                \textbf{Ours} & \textbf{\name{} + \tabqa{}} & \textbf{45.2} \\
                \bottomrule
            \end{tabular}
        }
    \end{center}
    \caption{Comparison of relieved accuracy scores for TabVQA tasks on FinTabNetQA, highlighting the best score achieved by our proposed approach (\name{} + \tabqa), showing an improvement of 9.2\% over the strongest baseline.}
    \label{table:fintabnetqa_scores}
\end{table}


\begin{figure*}
    \centering
    \includegraphics[width=0.9\linewidth]{sec/figures/DELTA-Qual.pdf}
    \caption{An example illustrating TabVQA for a table image from the FinabNetQA dataset, highlighting the OTSL string provided by \name{} and the answer produced by \tabqa. The predicted answer matches the actual answer from the ground truth.}
    \label{fig:qual}
\end{figure*}


\section{Conclusion}
\label{sec:conclusion}
In summary, we present a comprehensive pipeline for table understanding and reasoning. We begin with \name, a decoupled table reconstruction framework that separates structure recognition from OCR, producing a compact OTSL representation. \name{} achieves high TEDS-S scores and outperforms recent VLM-based approaches on standard benchmarks. To bridge the gap between widely used structured outputs and downstream reasoning tasks, we introduce an effective and lossless HTML-to-OTSL conversion algorithm. Finally, we propose \tabqa, an LLM fine-tuned on OTSL-formatted tables for the TabVQA task. \tabqa{} demonstrates superior performance compared to other models trained using different paradigms, achieving strong results on benchmarks like WTQ and FinTabNetQA. Collectively, these contributions define a flexible and extensible framework for high-fidelity table reconstruction and reasoning over structured tabular data.
\label{sec:Conclusion}

\section{Limitations and Future Work}
\label{sec:future}
While \name{} demonstrates good TEDS-S scores, the overall TEDS scores can still be improved. This is due to the current OCR support in the pipeline, which introduces errors that not only affect the TEDS score but can also impact downstream performance, particularly in content-sensitive tasks. Secondly, our experiments on table reconstruction and question answering have been conducted exclusively on English-language benchmarks, limiting the system’s applicability to multilingual or low-resource document settings. However, given the modular design of our framework, support can be extended to other languages in a straightforward manner, requiring only the replacement of the OCR and LLM components with multilingual or language-specific alternatives. Looking ahead, we also aim to incorporate multilingual datasets and evaluate performance across a broader spectrum of scripts and languages. Furthermore, we plan to enhance the reasoning capabilities of our system by supporting more complex queries, including abstract question answering and reasoning over densely populated or nested tables. These directions offer promising opportunities to broaden the scope and impact of our approach.
\label{sec:Future}



==> R1_Archive/sec/apendix.tex <==
% \section{Appendix}
% \label{sec:Appendix}

% \newpage

% \textcolor{red}{needs to be change according to our hyperparameter}
% \begin{table}[htbp]
% \centering
% \caption{Hyperparameters used during pre-training and fine-tuning}
% \begin{tabular}{lcc}
% \hline
% \textbf{Hyperparameter}     & \textbf{Pre-training} & \textbf{Fine-tuning} \\
% \hline
% Training steps              & 415                   & -- \\
% Number of epochs            & 5                     & -- \\
% \multicolumn{2}{l}{Batch size}               & 128 \\
% \multicolumn{2}{l}{Optimizer}                & AdamW \\
% \multicolumn{2}{l}{Learning rate}            & 2.00E-04 \\
% \multicolumn{2}{l}{Learning rate decay}      & Linear \\
% \multicolumn{2}{l}{Adam $\beta$}             & (0.9, 0.98) \\
% \multicolumn{2}{l}{Weight decay}             & 0.01 \\
% \multicolumn{2}{l}{Dropout}                  & 0.1 \\
% \hline
% \end{tabular}
% \end{table}

